Fast and Scalable Sparse Triangular Solver for Multi-GPU Based HPC Architectures

Designing efficient and scalable sparse linear algebra kernels on modern multi-GPU based HPC systems is a daunting task due to significant irregular memory references and workload imbalance across the GPUs. This is particularly the case for Sparse Triangular Solver (SpTRSV) which introduces additional two-dimensional computation dependencies among subsequent computation steps. Dependency information is exchanged and shared among GPUs, thus warrant for efficient memory allocation, data partitioning, and workload distribution as well as fine-grained communication and synchronization support. In this work, we demonstrate that directly adopting unified memory can adversely affect the performance of SpTRSV on multi-GPU architectures, despite linking via fast interconnect like NVLinks and NVSwitches. Alternatively, we employ the latest NVSHMEM technology based on Partitioned Global Address Space programming model to enable efficient fine-grained communication and drastic synchronization overhead reduction. Furthermore, to handle workload imbalance, we propose a malleable task-pool execution model which can further enhance the utilization of GPUs. By applying these techniques, our experiments on the NVIDIA multi-GPU supernode V100-DGX-1 and DGX-2 systems demonstrate that our design can achieve on average 3.53x (up to 9.86x) speedup on a DGX-1 system and 3.66x (up to 9.64x) speedup on a DGX-2 system with 4-GPUs over the Unified-Memory design. The comprehensive sensitivity and scalability studies also show that the proposed zero-copy SpTRSV is able to fully utilize the computing and communication resources of the multi-GPU system.

==> sec-discussion.tex <==

\section{Discussion}
\textbf{Extending to Multi-Nodes Multi-GPU Systems.}
Our proposed work aims to provide the ``scale-up" solution for today's supercomputer systems, thus targeting the state-of-the-art single-node multi-GPUs platforms which have been widely adopted in top500 and exascale systems. They are often seen as a good representation of what future heterogeneous architectures may look like, in comparison with the traditional sense of distributed designs via external interconnects. However, the proposed approach can be easily extended to the traditional distributed multi-node systems to ``scale-out". Firstly, NVSHMEM which enables fine-grained inter-GPU communication inside CUDA kernels can be translated to GPU RDMA massage passing by the network hardware or to LD/STs on fabrics like NVLinks. It also supports the multi-node system if GPUs are directly connected. Secondly, previous works such as GPUrdma\cite{daoud2016gpurdma} and GIO\cite{dGPU2020} either involve the CPU in the critical path or propose an intra-kernel PGAS programming model to enable GPUs to communicate directly for multi-node systems. Combining these communication channels inside our SpTRSV kernel, the proposed algorithm and read-only inter-GPU communication module can also be used in multi-node multi-GPU systems where GPUs are not point-to-point connected. Finally, the proposed SpTRSV kernel for single-node multi-GPU systems is orthogonal to the existing works that exploit parallelism on multi-node systems by partitioning and distributing less dependent data on distributed memory \cite{bauer2012legion,bauer2019legate,lee2019constraint,cojean2019resource, ben2019stateful}. After pre-processing and pre-allocating the matrices as sub-tasks for each node, our approach can speedup the parallel execution which leads to the overall performance improvement. 

%\vspace{4pt} \noindent \textbf{Workload Distribution in Exascale Machines.} To exploit parallelism on distributed memory systems, orchestrated data partitioning and distribution have been proposed by a variety of existing works \cite{bauer2012legion,bauer2019legate,lee2019constraint,cojean2019resource, ben2019stateful}. Bauer et al. propose the "\emph{Legion}" programming model to initiate independent tasks for exascale machines \cite{bauer2012legion}. They further propose a dynamic control mechanism for mapping NumPy Python programs \cite{bauer2019legate}. Lee et al.\cite{lee2019constraint} present a constraint-based approach that can automatically partition and distribute data among execution nodes. None of these works, however, have discussed the SpTRSV kernel which incurs massive irregular data dependency. To the best of our knowledge, this is the first work discussing how to efficiently implement SpTRSV for a multi-GPU system.



\textbf{Enabling Fast and Scalable Communication for Other Problems.}
Since SpTRSV often serves as an essential component for a linear-algebra solver/system/task\cite{vuduc2002automatic,vuduc2003automatic,mayer2009parallel, wolf2010factors,wang2018,Sao2019,ding2020leveraging,acceleration2016,SpTRSV2018grid}, we assume the data has already been stored across multi-GPUs. We then focus on the multi-GPU design for highly efficient SpTRSV. This is different from conventional scale-up solutions where data sharing can be achieved through CPU-based methodologies like MPI, global array, etc. Our experience from designing the new SpTRSV can guide the research into other irregular kernels such as \textit{matrix decomposition and transposition} on current and future multi-accelerator based heterogeneous systems. For example, NVSHMEM, the one-sided communication inside CUDA kernels, can be used to replace the send-receive interface that is widely used for GPU-to-GPU communication to further reduce the synchronization overhead. Our \textit{read-only communication approach} can also be leveraged to update the intermediate values locally without lock-spin synchronization and system-wide atomic operations. Finally, our task composition and scheduling can be further explored to solve more general problems (e.g., SpMV, SpGEMM and sparse tensor operations) under a multi-accelerator system for better workload balancing.    






